Improving Respiratory Sound Classification with Architecture-Agnostic Knowledge Distillation from Ensembles

Respiratory sound datasets are limited in size and quality, making high performance difficult to achieve. Ensemble models help but inevitably increase compute cost at inference time. Soft label training distills knowledge efficiently with extra cost only at training. In this study, we explore soft labels for respiratory sound classification as an architecture-agnostic approach to distill an ensemble of teacher models into a student model. We examine different variations of our approach and find that even a single teacher, identical to the student, considerably improves performance beyond its own capability, with optimal gains achieved using only a few teachers. We achieve the new state-of-the-art Score of 64.39 on ICHBI, surpassing the previous best by 0.85 and improving average Scores across architectures by more than 1.16. Our results highlight the effectiveness of knowledge distillation with soft labels for respiratory sound classification, regardless of size or architecture.

==> Tables/_deprecated_soft_hard_comp.tex <==

\begin{table*}[!t]

    \caption{Overall comparison of hard and soft labels on the ICBHI dataset for the official 60--40\% train--test split task of respiratory sound classification. \emph{All of the checkpoints are implemented and reproduced for this work.}}
    
    \label{tab:soft_hard_comp}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{llll|lll|lll}
             &\multicolumn{3}{c}{Hard Label}    &\multicolumn{3}{c}{Soft Label}    &\multicolumn{3}{c}{Gain} \\
Model        & Sp           & Se           & Score        & Sp           & Se           & Score        & Sp          & Se           & Score       \\
CNN6         & 80.20 ± 2.70 & 35.87 ± 3.21 & 58.04 ± 0.56 & 85.57 ± 2.56 & 30.77 ± 1.97 & 58.17 ± 0.60 & 5.37 & -5.10 & 0.14  \\
EfficientNet & 76.50 ± 3.85 & 35.19 ± 1.85 & 55.85 ± 1.19 & 79.26 ± 3.31 & 36.09 ± 3.39 & 57.68 ± 1.48 & 2.76 & 0.90  & 1.83  \\
Resnet18     & 76.54 ± 4.09 & 32.59 ± 3.61 & 54.57 ± 0.53 & 81.41 ± 2.78 & 31.11 ± 3.05 & 56.26 ± 0.85 & 4.87 & -1.48 & 1.69  \\
AST          & 77.69 ± 2.72 & 42.97 ± 3.22 & 60.33 ± 0.82 & 79.24 ± 3.51 & 42.92 ± 4.04 & 61.08 ± 1.26 & 1.55 & -0.05 & 0.75  \\
Audio-CLAP   & 80.85 ± 3.33 & 44.67 ± 3.77 & 62.56 ± 0.37 & 82.82 ± 2.14 & 44.44 ± 2.35 & 63.63 ± 0.60 & 1.97 & -0.23 & 1.07  \\
BTS          & 82.81 ± 2.26 & 43.70 ± 1.83 & 63.26 ± 0.57 & 82.89 ± 2.14 & 45.90 ± 1.89 & 64.39 ± 0.42 & 0.08 & 2.19  & 1.13  \\
\midrule
Mean         &              &              &              &              &              &              &2.77 & -0.63 & 1.10
\end{tabular}
}
    %\vspace{5mm}
\end{table*}

==> Tables/ablations.tex <==
\begin{table}[]
 \caption{Ablation Study}
    \label{tab:ablations}
\begin{tabular}{l|lll}
Method           & S\_p         & S\_e         & Score        \\
Baseline         & 82.81 ± 2.26 & 43.70 ± 1.83 & 63.26 ± 0.57 \\
Noised Label (var)     & 76.53 ± 3.78 & 47.46 ± 2.36 & 62.00 ± 1.06 \\
Noised Label (var \& bias)     & \multicolumn{3}{c}{Failed to converge} \\
Single Teacher      & 83.18 ± 1.59 & 44.62 ± 1.56 & 63.90 ± 0.15\\
Teacher Ensemble    & 82.89 ± 2.14 & 45.90 ± 1.89 & 64.39 ± 0.42  \\
Remove softmax    & \multicolumn{3}{c}{Failed to converge}
\end{tabular}
\end{table}
